Operation-based Refactoring-aware Merging: An Empirical Evaluation

Dealing with merge conflicts in version control systems is a challenging task for software developers. Resolving merge conflicts is a time-consuming and error-prone process, which distracts developers from important tasks. Recent work shows that refactorings are often involved in merge conflicts and that refactoring-related conflicts tend to be larger, making them harder to resolve. In the literature, there are two refactoring-aware merging techniques that claim to automatically resolve refactoring-related conflicts; however, these two techniques have never been empirically compared. In this paper, we present RefMerge, a rejuvenated Java-based design and implementation of the first technique, which is an operation-based refactoring-aware merging algorithm. We compare RefMerge to Git and the state-of-the-art graph-based refactoring-aware merging tool, IntelliMerge, on 2,001 merge scenarios with refactoring-related conflicts from 20 open-source projects. We find that RefMerge resolves or reduces conflicts in 497 (25%) merge scenarios while increasing conflicting LOC in only 214 (11%) scenarios. On the other hand, we find that IntelliMerge resolves or reduces conflicts in 478 (24%) merge scenarios but increases conflicting LOC in 597 (30%) merge scenarios. We additionally conduct a qualitative analysis of the differences between the three merging algorithms and provide insights of the strengths and weaknesses of each tool. We find that while IntelliMerge does well with ordering and formatting conflicts, it struggles with class-level refactorings and scenarios with several refactorings. On the other hand, RefMerge is resilient to the number of refactorings in a merge scenario, but we find that RefMerge introduces conflicts when inverting move-related refactorings.

==> tables/extratabs.tex <==
\begin{table*}[t]
\caption{}
\centering
\addtolength{\tabcolsep}{0.25cm}
\resizebox{1\textwidth}{!}{
\begin{tabular}[width=\textwidth]{lrrrrrrrr}
\toprule
\multirow{2}{*}{\textbf{Project}} & \multirow{2}{*}{\textbf{Total Scenarios}} & \multicolumn{3}{c}{\textbf{IntelliMerge}} & \multicolumn{3}{c}{\textbf{RefMerge}}\\
\cmidrule(lr){3-5}
\cmidrule(lr){6-8}
&&{\makecell{\textbf{Completely} \\ \textbf{Resolved} \\
\textbf{Scenarios}}}& \makecell{\textbf{Conflicting} \\ \textbf{Scenarios}}& \makecell{\textbf{Timed Out} \\ \textbf{Scenarios}} 

&{\makecell{\textbf{Completely} \\ \textbf{Resolved} \\
\textbf{Scenarios}}}& \makecell{\textbf{Conflicting} \\ \textbf{Scenarios}}& \makecell{\textbf{Timed Out} \\ \textbf{Scenarios}}\\
% &{\textbf{Git}}&\textbf{\ourtool}&\textbf{IntelliMerge}&{\textbf{Git}}&\textbf{\ourtool}&\textbf{IntelliMerge}\\

\midrule
cassandra& \checkNum{535} & \checkNum{33} & \checkNum{21} & \checkNum{481} & \checkNum{15} & \checkNum{172} & \checkNum{365}  \\ 
elasticsearch& 178 & 3 (2\%)& 104 (58\%) & 71 & 8 & 153 & 17 \\
gradle& 117 & 1 & 111 & 6 & 10 & 108 & 0 \\
antlr4& 100 & 1 & 96 & 3 & 1 & 0 & 99 \\
platform\_frameworks\_support& 96 & 5 & 58 & 33 & 7 & 89 & 0 \\
deeplearning4j& 93 & 3 & 89 & 1 & 5 & 88 & 0 \\ 
realm-java& 92 & 7 & 83 & 2 & 8 & 84 & 0\\
jackson-core& 81 & 0 & 81 & 0 & 3 & 78 & 0\\
android& 81 & 3 & 78 & 0 & 8 & 73 & 0\\
cometd& 63 & 2 & 60 & 1 & 5 & 58 & 0 \\
storm& 33 & 1 & 32 & 0 & 0 & 33 & 0 \\
ProjectE& 30 & 1 & 28 & 1 & 0 & 30 & 0 \\
javaparser& 23 & 3 & 20 & 0 & 0 & 23 & 0 \\
druid& 17 & 2 & 15 & 0 & 1 & 16 & 0\\
androidannotations& 15 & 1 & 14 & 0 & 0 & 15 & 0\\
junit4& 14 & 1 & 13 & 0 & 1 & 13 & 0 \\
MinecraftForge& 14 & 2 & 10 & 2 & 0 & 14 & 0 \\
iFixitAndroid& 13 & 0 & 13 & 0 & 1 & 12 & 0\\
MozStumbler& 10 & 0 & 10 & 0 & 1 & 9 & 0 \\
error-prone& 9 & 1 & 8 & 0 & 0 & 0 & 9 \\
\midrule
Total & \checkNum{1,614} & \checkNum{70} & \checkNum{944} & \checkNum{600} & \checkNum{74} & \checkNum{1175} & \checkNum{365} \\
\bottomrule
\end{tabular}
}
\label{tab:conflict-scenarios}
\vspace{-4mm}
\end{table*}

==> tables/tab-conflict-change.tex <==
\begin{table*}[t]
\caption{Number of merge scenarios with reduced/increased conflicting files, conflicting blocks, and conflicting lines of code (LOC). Note that this number of scenarios does \textbf{not} include completely resolved scenarios. This table focuses on scenarios that were not resolved but for which the conflict result changes at one of the conflict granularity levels. The number in parentheses shows the median percentage reduction/increase per merge scenario in that project.}
\centering
\addtolength{\tabcolsep}{0.25cm}
\resizebox{1\textwidth}{!}{
\begin{tabular}[width=\textwidth]{lrrrrrrrrrrrr}
\toprule
\multirow{3}{*}{\textbf{Project}} & \multicolumn{4}{c}{\textbf{Conflicting Files}} & \multicolumn{4}{c}{\textbf{Conflict Blocks}} & \multicolumn{4}{c}{\textbf{Conflicting LOC}} \\
\cmidrule(lr){2-5}
\cmidrule(lr){6-9}
\cmidrule(lr){10-13}
& \multicolumn{2}{c}{\textbf{IntelliMerge}} & \multicolumn{2}{c}{\textbf{RefMerge}} & \multicolumn{2}{c}{\textbf{IntelliMerge}} & \multicolumn{2}{c}{\textbf{RefMerge}} & \multicolumn{2}{c}{\textbf{IntelliMerge}} & \multicolumn{2}{c}{\textbf{RefMerge}} \\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-7}
\cmidrule(lr){8-9}
\cmidrule(lr){10-11}
\cmidrule(lr){12-13}
& \textbf{Reduced} & \textbf{Increased}  & \textbf{Reduced} & \textbf{Increased}  & \textbf{Reduced} & \textbf{Increased} &  \textbf{Reduced} & \textbf{Increased} & \textbf{Reduced} & \textbf{Increased} & \textbf{Reduced} & \textbf{Increased} \\

% \cmidrule(lr){3-5}
% \cmidrule(lr){6-8}
% &&{\makecell{\textbf{Completely} \\ \textbf{Resolved} \\
% \textbf{Scenarios}}}& \makecell{\textbf{Conflicting} \\ \textbf{Scenarios}}& \makecell{\textbf{Timed Out} \\ \textbf{Scenarios}} 

% &{\makecell{\textbf{Completely} \\ \textbf{Resolved} \\
% \textbf{Scenarios}}}& \makecell{\textbf{Conflicting} \\ \textbf{Scenarios}}& \makecell{\textbf{Timed Out} \\ \textbf{Scenarios}} \\
% & 
% &{\textbf{Git}}&\textbf{\ourtool}&\textbf{IntelliMerge}&{\textbf{Git}}&\textbf{\ourtool}&\textbf{IntelliMerge}\\

\midrule
cassandra& \checkNum{0 (0\%)} & \checkNum{730 (329\%)} & \checkNum{72 (33\%)} & \checkNum{120 (33\%)} & \checkNum{0 (0\%)} & \checkNum{21 (450\%)} & \checkNum{0 (0\%)} & \checkNum{10 (15\%)} & \checkNum{2 (31\%)} & \checkNum{19 (164\%)} & \checkNum{0 (0\%)} & \checkNum{0 (0\%)}\\ 
elasticsearch& 4 (20\%) & 99 (260\%) & 15 (33\%) & 24 (55\%) & 4 (28\%) & 95 (271\%) & 22 (33\%) & 35 (25\%) & 38 (45\%) & 65 (118\%) & 48 (17\%) & 41 (28\%) \\
gradle& 6 (33\%) & 91 (500\%) & 10 (22\%) & 14 (50\%) & 10 (33\%) & 95 (433\%) & 18 (19\%) & 20 (45\%) & 38 (45\%) & 73 (190\%) & 33 (19\%) & 28 (47\%) \\
antlr4& 2 (56\%) & 92 (445\%) & 6 (18\%) & 15 (17\%) & 3 (20\%) & 92 (479\%) & 7 (5\%) & 21 (13\%) & 20 (27\%) & 75 (102\%) & 23 (4\%) & 39 (10\%) \\
platform\_frameworks\_support& 5 (70\%) & 44 (375\%) & 5 (4\%) & 9 (18\%) & 8 (51\%) & 47 (517\%) & 9 (25\%) & 16 (13\%) & 24 (58\%) & 33 (130\%) & 27 (16\%) & 24 (10\%) \\
deeplearning4j& 6 (67\%) & 59 (160\%) & 0 (0\%) & 9 (80\%) & 20 (42\%) & 63 (175\%) & 6 (9\%) & 13 (29\%) &??&??&??&?? \\ 
realm-java& 10 (39\%) & 46 (181\%) & 4 (25\%) & 5 (50\%) & 22 (50\%) & 47 (200\%) & 13 (21\%) & 7 (40\%) & 45 (45\%) & 43 (148\%) & 13 (10\%) & 15 (20\%) \\
jackson-core& 0 (0\%) & 79 (850\%) & 6 (33\%) & 11 (50\%) & 0 (0\%) & 80 (1522\%) & 11 (33\%) & 17 (38\%) & 8 (47\%) & 72 (430\%) & 20 (9\%) & 22 (42\%) \\
android& 6 (38\%) & 55 (167\%) & 2 (30\%) & 1 (10\%) & 21 (40\%) & 52 (124\%) & 3 (17\%) & 9 (33\%) & 54 (58\%) & 23 (119\%) & 10 (6\%) & 7 (44\%) \\
cometd& 2 (47\%) & 48 (658\%) & 3 (25\%) & 3 (8\%) & 3 (23\%) & 52 (809\%) & 6 (25\%) & 5 (11\%) & 15 (51\%) & 43 (241\%) & 9 (24\%) & 10 (9\%) \\
storm& 3 (33\%) & 22 (345\%) & 1 (33\%) & 1 (100\%) & 3 (25\%) & 26 (233\%) & 4 (25\%) & 1 (6\%) & 14 (39\%) & 16 (119\%) & 9 (30\%) & 1 (1\%) \\
ProjectE& 4 (12\%) & 24 (79\%) & 2 (45\%) & 6 (7\%) & 4( 15\%) & 22 (94\%) & 4 (20\%) & 8 (11\%) & 18 (45\%) & 10 (75\%) & 13 (11\%) & 9 (9\%) \\
javaparser& 5 (43\%) & 8 (150\%) & 4 (59\%) & 3 (50\%) & 3 (90\%) & 10 (369\%) & 5 (80\%) & 4 (21\%) & 12 (59\%) & 7 (275\%) & 6 (40\%) & 7 (21\%) \\
druid& 8 (46\%) & 0 (0\%) & 2 (33\%) & 1 (50\%) & 13 (67\%) & 0 (0\%) & 6 (50\%) & 3 (8\%) & 15 (85\%) & 0 (0\%) & 10 (7\%) & 1 (57\%) \\
androidannotations& 1 (67\%) & 13 (100\%) & 3 (50\%) & 1 (10\%) & 1 (89\%) & 13 (114\%) & 2 (58\%) & 2 (17\%) & 4 (87\%) & 10 (42\%) & 6 (37\%) & 6 (46\%) \\
junit4& 5 (33\%) & 7 (150\%) & 0 (0\%) & 5 (50\%) & 5 (60\%) & 7 (233\%) & 0 (0\%) & 5 (25\%) & 10 (65\%) & 3 (18\%) & 3 (6\%) & 5 (33\%) \\
MinecraftForge& 1 (10\%) & 9 (100\%) & 1 (17\%) & 2 (149\%) & 1 (5\%) & 9 (100\%) & 3 (19\%) & 3 (33\%) & 4 (27\%) & 4 (150\%) & 4 (13\%) & 4 (58\%) \\
iFixitAndroid& 5 (81\%) & 5 (78\%) & 4 (93\%) & 3 (1500\%) & 6 (57\%) & 7 (100\%) & 3 (96\%) & 4 (583\%) & 7 (34\%) & 5 (55\%) & 4 (78\%) & 5 (74\%) \\
MozStumbler& 1 (25\%) & 5 (50\%) & 2 (37\%) & 1 (20\%) & 3 (50\%) & 5 (86\%) & 4 (24\%) & 2 (21\%) & 7 (56\%) & 3 (38\%) & 5 (34\%) & 2 (17\%) \\ 
error-prone& 4 (46\%) & 3 (750\%) & 2 (25\%) & 0 (0\%) & 2 (91\%) & 5 (417\%) & 3 (33\%) & 0 (0\%) & 3 (84\%) & 5 (187\%) & 3 (33\%) & 4 (65\%) \\
\midrule
Total & \checkNum{78 (40\%)} & \checkNum{730 (329\%)} & \checkNum{72 (33\%)} & \checkNum{120 (33\%)} & \checknum{132 (50\%)} & \checknum{748 (363\%)} & \checknum{129 (25\%)} & \checknum{185 (25\%)} & \checknum{391 (51\%)} & \checknum{538 (161\%)} & \checknum{266 (13\%)} & \checkNum{237 (23\%)} \\
\bottomrule
\end{tabular}
}
\label{tab:conflict-change}
\end{table*}


==> tables/tab-full-conflscen-stats.tex <==
\begin{table*}[t]
\caption{Statistics for each of the 20 open-source projects that we evaluate on. The Git column shows the number of conflicting merge scenarios with involved refactorings, as reported by git through Mahmoudi et al.'s tooling~\cite{SANER}. These are the merge scenarios we consider in our evaluation. The 10 projects in the IntelliMerge paper are shown in bold. 
The remaining two columns show the number of conflicting scenarios reported by each tool. When a tool reports less conflicts than git, we include the percent reduction in parentheses. The  merge  tool  that  reports  the  least conflicting  merge  scenarios  for  each  project  is  marked  in bold.}
\centering
\addtolength{\tabcolsep}{0.25cm}
\resizebox{0.7\textwidth}{!}{
\begin{tabular}[width=\textwidth]{lrrrrr}
\toprule
\multirow{2}{*}{\textbf{Project}} & \multirow{2}{*}{\textbf{Stargazers}} & \multicolumn{3}{c}{\textbf{Number of Conflicting Merge Scenarios}}\\
\cmidrule(lr){3-5}
&&{\textbf{Git}}&\textbf{\ourtool}&\textbf{IntelliMerge}\\
% &{\textbf{Git}}&\textbf{\ourtool}&\textbf{IntelliMerge}&{\textbf{Git}}&\textbf{\ourtool}&\textbf{IntelliMerge}\\

\midrule
\textbf{cassandra}& 6,882 &922&\checkNum{329} & \checkNum{305} \\ 
\textbf{elasticsearch}& 56,665 &178& \textbf{170 (4.5\%)} & 175 (1.69\%)  \\
\textbf{gradle}& 12,410 &117& \textbf{108 (7.69\%)} & \117 \\
\textbf{antlr4}& 10,738 &100 & \textbf{99 (1\%)} & \textbf{99 (1\%)}\\
platform\_frameworks\_support& 1,609 & 96 & 87 (9.38\%) & \textbf{81 (15.63\%)} \\
\textbf{deeplearning4j}& 12,208 & 93 & \textbf{88 (5.38\%)} & 90 (3.23\%)\\
\textbf{realm-java}& 11,206 &92 & \textbf{84 (8.70\%)} & 85 (7.61\%)\\
jackson-core& 1,984 & 81 &\textbf{78 (3.70\%)} & 81\\
android& 3,161 & 81 & \textbf{73 (9.88\%)} & 78 (3.70\%) \\
cometd& 535 & 63 & \textbf{58 (7.94\%)} & 61 (3.17\%)\\
\textbf{storm}& 6,278 &33 &33 & \textbf{32 (3.03\%)}\\
ProjectE& 308 & 30 & 30 & \textbf{29 (3.33\%)}  \\
\textbf{javaparser}& 3,859 &23 &23 & \textbf{20 (13.04\%)} \\
druid& 24,576 & 17& 16 (5.88\%) & \textbf{15 (11.77\%)} \\
androidannotations& 11,171 & 15 & 15 & \textbf{14 (6.67\%)} \\
\textbf{junit4}& 8,198 & 14& \textbf{13 (7.14\%)} & \textbf{13 (7.14\%)} \\
MinecraftForge& 4,945 & 14 & 14 & \textbf{12 (14.28\%)} \\
iFixitAndroid& 143 & 13& \textbf{12 (7.69\%)} & 13 \\
MozStumbler& 609 & 10& \textbf{9 (10\%)} & 10 \\
\textbf{error-prone}& 5,717 &9 & 9 & \textbf{8 (11.11\%)} \\
\midrule
Total &  & 2,002& \checkNum{\textbf{1,347 (4.41\%)}} & \checkNum{\textbf{1,347 (4.41\%)}}\\
Median&&&\todo{X}&\todo{Y}\\
\bottomrule
\end{tabular}
}
\label{tab:conflict-scenarios}
\vspace{-4mm}
\end{table*}

==> tables/tab-overall-scenario-details.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[t]
\centering
\caption{\revision{Breakdown of merge scenarios for each project.}}
\label{tab:scenario-details}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{@{}lr
>{\raggedleft\arraybackslash}p{3.5cm}
>{\raggedleft\arraybackslash}p{3.5cm}
>{\raggedleft\arraybackslash}p{3.5cm}
@{}}
\toprule
\textbf{Project Name} & \textbf{Total Scenarios} & \textbf{Scenarios with only refactoring-involved conflicts} & \textbf{} & \textbf{Median Changed Files} \\ 
\midrule
cassandra               & 922   &   244 & 1,462 & \\
elasticsearch           & 178   &   30  & 155   & \\
gradle                  & 118   &   28  & 152   & \\
antlr4                  & 100   &   14  & 461   & \\
platform\_fwk\_support    & 95    &   25  & 919   & \\
deeplearning4j          & 93    &   20  & 30    & \\
realm-java              & 92    &   23  & 56    & \\
jackson-core            & 81    &   17  & 401   & \\
android                 & 81    &   9   & 149   & \\
cometd                  & 63    &   11  & 133   & \\
storm                   & 33    &   12  & 122   & \\
ProjectE                & 30    &   3   & 89    & \\
javaparser              & 23    &   6   & 19    & \\
druid                   & 17    &   3   & 2     & \\
androidannotations      & 15    &   1   & 94    & \\
junit4                  & 14    &   2   & 36    & \\
MinecraftForge          & 14    &   3   & 53    & \\
iFixitAndroid           & 13    &   0   & 71    & \\
MozStumbler             & 10    &   1   & 52    & \\
error-prone             & 9     &   1   & 58    & \\
\midrule
Total                   & 2,001 & 453   &       & \\
\bottomrule
\end{tabular}
}
\vspace{-4mm}
\end{table*}

==> tables/tab-refactoring-logic.tex <==
% Commands for table cells
\newcommand{\vcell}[1]{\rotatebox[origin=c]{90}{#1}}

\begin{table*}
\centering
\bgroup
% \vspace{-0.5cm}
\def\arraystretch{1.2}
\caption{Conflict logic of supported refactorings}
\label{table:methods_mappings}
% \vspace{2mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccccccc}
\toprule
% Rename Method / Rename Method
% Move Method / Move Method
% Move And Rename Method / Move And Rename Method
% Rename Class / Rename Class
% Move Class / Move Class
% Move And Rename Class / Move And Rename Class
% Inline Method / Extract Method
% Extract Method / Inline Method
% Rename Field (Work In Progress) / Rename Field
& \vcell{\texttt{Rename Method(m$_1$, m$_2$)}} & \vcell{Move Method} & \vcell{Move \& Rename Method} & \vcell{Rename Class} & \vcell{Move \& Rename Class} & \vcell{Inline Method} & \vcell{Extract Method} & \vcell{Rename Field}\\
\midrule
\texttt{Rename Method(m$_3$, m$_4$)}&conflict = ($m_1 == m_3 \land m2 != m4$) \lor (m$_1$ != m$_3$ \land m$_2$ == m$\_4$)\\
Move Method&\\
Move and Rename Method&\\
Rename Class\\
Move and Rename Class\\
Inline Method\\
Extract Method\\
Rename Field\\
% \multicolumn{1}{|c|}{} & Argument Change & \cellcolor{myyellow}Potential Conflict & \cellcolor{myred}Conflict & \cellcolor{myyellow}Potential Conflict & \cellcolor{myred}Conflict \\ \hhline{|~|-|-|-|-|-}

% \multicolumn{1}{|c|}{} & Body-only & \cellcolor{myyellow}Potential Conflict & \cellcolor{myyellow}Potential Conflict & \cellcolor{myyellow}Potential Conflict & \cellcolor{myred}Conflict \\ \hhline{|~|-|-|-|-|-}

% \multicolumn{1}{|c|}{} & Deleted & \cellcolor{myred}Conflict & \cellcolor{myred}Conflict & \cellcolor{myred}Conflict & \cellcolor{mygreen}No Conflict \\ \hhline{|-|-|-|-|-|-}

\end{tabular}
}
\egroup
\end{table*}
